Compact schemes for laser-matter interaction in Schr\"odinger equation

Numerical solutions for laser-matter interaction in Schr\"odinger equation has many applications in theoretical chemistry, quantum physics and condensed matter physics. In this paper we introduce a methodology which allows, with a small cost, to extend any fourth-order scheme for Schr\"odinger equation with time-indepedent potential to a fourth-order method for Schr\"odinger equation with laser potential. These fourth-order methods improve upon many leading schemes of order six due to their low costs and small error constants.

==> S2_FirstMethod.tex <==
Following the approach of \cite{BIKS,IKS18sinum}, the \schr equation
\R{eq:schr} can be written in the form
\begin{equation}\label{eq:Amag}
 u'(t)= A(t) u(t),\qquad t\geq0,
\end{equation}
with $A(t) = \ii [\ve \dx^2 -  \ve^{-1} V(t)]$. Its solution can be
approximated via the Magnus expansion \cite{magnus54}, which is an infinite
series of nested integrals and commutators. In practice we use finite
truncations of this series for a numerical scheme,
\begin{equation}\label{eq:Amag2}
u^{n+1} = \ee^{\Theta_m(t_{n+1},t_n)} u^n,
\end{equation}
where $t_n = t_0 + n\dt$, $\dt$ is the time step, $u^n$ is an approximation
to the exact solution at $t_n$, and $\Theta_m(t,s)$ is a finite truncation of
the Magnus expansion $\Theta(t,s)$ whose exponential evolves the exact solution from $s$
to $t$.

\subsection{Simplified-commutator Magnus expansions}
In the semiclassical regime, the order two and order four
simplified-commutator Magnus expansions of \cite{IKS18sinum} that preserve
the integral become
\begin{Eqnarray*}
\label{eq:Omt1} \Theta_0(h) &=& \ii \dt \ve \dx^2 - \ii  \ve^{-1} \momO,\\
\label{eq:Omt3} \Theta_2(h) &=& \ii \dt \ve \dx^2 - \ii  \ve^{-1} \momO -
2\Ang{1}{\dx \mom{1}{1}},
\end{Eqnarray*}
respectively.  This follows directly from the results of \cite{IKS18sinum}
by accounting for the additional scalar factors  $\ve$ and $\ve^{-1}$. The quantities $\momO$ and $\mom{1}{1}$ have been already  introduced
earlier and
\begin{equation}\label{eq:angbra}
  \ang{f}{k} := \Frac12 \left( f \circ \dx^k + \dx^k \circ f \right), \quad  k \geq 0,\ f \in
  \CC{C}_p^{\infty}(I;\BB{R})
\end{equation}
are the symmetrised differential operators which first appeared in
\cite{bader14eaf}, and have been studied in detail in
\cite{psalgebra,Singh17}. These operators are used here for the same reasons as in \cite{bader14eaf,BIKS,IKS18sinum} -- namely, for
preservation of stability under discretisation after simplification of
commutators.
%
%The semiclassical regime is characterised by the $\O{\ve}$ wavelength
%spatio-temporal oscillations that appear in the solution regardless of the
%smoothness of the initial conditions \cite{bao02ots,thesis}. In order to
%correctly resolve these oscillations, we require
%\begin{equation}
%\label{eq:Nve} N = \O{\ve^{-1}}
%\end{equation}
%spatial grid points \cite{bao02ots}, which can be very large. Consequently,
%the discretised\footnote{Throughout this manuscript we use the notation
%$\mathcal{L} \leadsto L$ to denote spatial discretisation of an operator
%$\mathcal{L}$ to the matrix $L$.} differentiation matrices are often very
%large in spectral radius,
%\begin{equation}
%\label{eq:dxve}
%\dx^k \leadsto \K_k = \O{N^k} =
%\O{\ve^{-k}}, \end{equation}
%\[ \Theta_m(h) = \O{h \ve^{-1}}\]
%due to the scaling of the leading term $\ii \dt \ve \dx^2$ alone. %Thus  Magnus expansion
%%via Lanczos iterations becomes expensive unless the time step is sufficiently depressed since
%Thus Lanczos based methods including \cite{IKS18sinum}, which are effective
%in the atomic scaling where $\ve=1$, become ineffective unless
%the time step is sufficiently depressed or iterations are increased. In either case, the cost grows prohibitively.


%\[ N = \O{\ve^{-1}}, \quad \dx^k \leadsto \K_k = \O{N^k} = \O{\ve^{-k}} \]
%For the purpose of this paper and for simplicity sake we assume that they
%belong to $\CC{C}_p^\infty(I; \BB{R})$ and $\CC{C}_p^\infty(I; \BB{C})$,
%respectively, the spaces of real valued and complex valued smooth periodic
%functions over $I$, but our results extend in a straightforward manner to
%functions of lower smoothness (the regularity constraints will depend on the
%desired order of the method being derived).
%
%\begin{equation}
%\label{eq:Omt3} \Theta_2(h) = \ii \dt \ve \dx^2 - \ii  \ve^{-1} \momO -
%2\Ang{1}{\dx \mom{1}{1}}
%\end{equation}
%where


\subsection{Analysis of size}
As a consequence of \R{eq:dxve}, the symmetrised differential operators scale
as
\begin{equation}\label{eq:angbradisc}
 \ang{f}{k} \leadsto \Frac12 \left( \DDD_f \K_k + \K_k \DDD_f \right) = \O{\ve^{-k}}
\end{equation}
upon discretisation, assuming that $f$ is independent of $\ve$. For
convenience, we abuse notation\footnote{This notion can be made more rigorous
by noting that in the semiclassical regime the derivatives of the solution
grow as $\norm{2}{\dx^k u}\leq C_k \ve^{-k}$, and consequently
$\norm{2}{\ang{f}{k}(u)} \leq C_k \norm{}{f} \ve^{-k}$. The analysis of the
methods presented here can be made rigorous in accordance with these
observations. See \cite{psalgebra,Singh17} for details. } somewhat and use
the shorthand $\ang{f}{k} = \O{\ve^{-k}}$ instead of \R{eq:angbradisc}.

%
%In numerically solving \R{eq:schr}, consistently with standard practice we
% impose periodic boundary conditions on a finite interval $I
%\subseteq \BB{R}$. We further assume throughout that the interaction
%potential $V(\cdot,t)$ and the wavefunction $u(\cdot,t)$ are sufficiently
%smooth.

%Also $\norm{2}{\ang{f}{k} u} = \O{\ve^{-k}}$ \cite{PSthesis}. All commutators
%are $\O{\ve^{-1}}$ or smaller (arXiv and thesis, also used in FoCM and BIKS).

\begin{theorem}\label{thm:ve}
All nested commutators of $\ve \dx^2$, $\ve^{-1} V$ and, in general, terms of
the form $\ve^{k} \ang{f}{k+1}$ are $\O{\ve^{-1}}$ or smaller
\cite{psalgebra,Singh17}.
\end{theorem}
Thus a grade $p$ (i.e. $p-1$ times nested) commutator  of $\ii h \ve \dx^2$
and $-\ii h \ve^{-1} V$, which is typically considered to be $\O{h^p}$,
without accounting for $\ve$ or growth corresponding to finer spatial
discretisation, becomes $\O{h^p \ve^{-1}}$ when analysed taking all factors
into account.

To unify the analysis of magnitude of terms, we express the time step in
terms of the inherent parameter $\ve$,
\begin{equation}\label{eq:hve} h = \O{\ve^{\sigma}},
\quad \sigma>0,
\end{equation}
where a smaller $\sigma$ corresponds to larger time steps. We will be aiming
to develop methods that work for small values of $\sigma$ and at the very
least we may assume that $\sigma \leq 1$.

Taylor expansion for an analytic potential, $V(\xi) = \sum_{k=0}^\infty
[V^{(k)}(0)/k!] \xi^k$, shows that $\mom{1}{1}=\int_0^\dt (\xi - h/2) V(\xi)
d\xi$ is $\O{h^3}$ for smooth potentials, since its $\O{h^2}$ term,
$V^{(0)}(0)\int_0^\dt (\xi - h/2) d\xi$, vanishes.

Combining all these ingredients, we conclude that
\begin{equation}
\label{eq:Omt3size}
\Theta_2(h) = \overbrace{\ii \dt \ve \dx^2}^{\O{\ve^{\sigma-1}}} - \overbrace{\ii  \ve^{-1} \momO}^{\O{\ve^{\sigma-1}}} -
\overbrace{2\Ang{1}{\dx \mom{1}{1}}}^{\O{\ve^{3\sigma-1}}}.
\end{equation}
Here it becomes evident that the two leading terms in the Magnus expansion
are significantly larger than the trailing terms. As mentioned in the
introduction, the direct usage of Lanczos iterations for $\exp(\Theta_2)$
 is costly due to the $\O{\ve^{\sigma-1}}$ growth of the
leading terms.

On the other hand, the large term $\ii \dt \ve \dx^2$ can be exponentiated
via FFTs at a $\O{N \log N}$ cost since it discretises as a circulant matrix
and the diagonal term $\ii \ve^{-1} \momO$ can be exponentiated directly at the cost of
$\O{N}$ operations. Thus, we resort to Zassenhaus splittings to separate these
vastly disparate scales, whereby only the small $\O{\ve^{3\sigma -1}}$ terms
need  be exponentiated via Lanczos iterations. The small size of the
remaining exponents means we can work with large time steps (a small
$\sigma$, say $\sigma=1/2$ for instance) and still require very few Lanczos
iterations.

\subsection{Symmetric Zassenhaus splitting of order four}

In order to split the exponential of the fourth-order Magnus expansion,
$\Theta_2$, using Zassenhaus splitting algorithm, we follow the procedure
outlined in Appendix~\ref{sec:Zassenhaus}. In particular, the exponential we
wish to approximate here is $\ee^{\Theta_2}$. Thus, we take
$\mathcal{W}^{[0]}=\Theta_{2}$, which needs to be split in two components, $X
= W^{[0]}$ and $Y = \mathcal{W}^{[0]}- W^{[0]}$. We usually prefer to extract
the largest terms first yet we may choose between $W^{[0]} = \ii \dt \ve
\dx^2$ and $W^{[0]} = -\ii \ve^{-1} \momO$, which are both
$\O{h\ve^{-1}}=\O{\ve^{\sigma-1}}$.

%\R{eq:definitionWW}

In the specific method presented here, we opt for the former,
whereby $X = W^{[0]}
= \ii \dt \ve \dx^2=\ii \dt \ve \ang{1}{2}$ and $Y = \mathcal{W}^{[0]}-
W^{[0]} =- \ii \ve^{-1} \ang{\momO}{0} - 2 \Ang{1}{\dx \mom{1}{1}}$. (Observe that $\ang{1}{k} = \dx^k$ and $\ang{f}{0} = f$. We
will switch between these  equivalent notations at our convenience.) Using
the sBCH formula \R{eq:sBCH}, we write
\begin{equation}\label{eq:3:sbch_inverted}
  \ee^{\Theta_{2}} = \ee^{\mathcal{W}^{[0]}} =\ee^{\frac12 \ii \dt \ve \dx^2} \ee^{\mathcal{W}^{[1]} } \ee^{\frac12  \ii \ve \dt \dx^2} + \O{h^5 \ve^{-1}},
\end{equation}
where, using the order four expression for $\mathcal{W}^{[1]} =
\CC{sBCH}(-X,X+Y)$ from \R{eq:sBCHshifted},
%\[ \mathcal{W}^{[1]} = \sBCH(- \ii \dt \dx^2, \mathcal{W}^{[0]}).\]
%Assuming $X=\O{h}$ and $Y=\O{h}$
%and substituting $-X$ for $X$ and $X+Y$ for $Y$ in the sBCH formula \R{eq:sBCHcoeffs}, the central exponent in \R{eq:3:sbch_inverted} is
%\begin{Eqnarray}
%\nonumber \mathcal{W}^{[1]} := \CC{sBCH}(-X,X+Y) &=& (-X + (X+Y)) - \Frac{1}{24}[[X+Y,X],X]\\
%\nonumber &&+\Frac{1}{12}[[X+Y,X],X+Y] \\
%%\nonumber &=& Y - \Frac{1}{24}[[Y,X],X] + \Frac{1}{12}[[Y,X],X+Y] +\O{\dt^5}\\
%\label{eq:sBCHshifted}&=&Y + \Frac{1}{24}[[Y,X],X] + \Frac{1}{12}[[Y,X],Y] ,
%\end{Eqnarray}
\begin{Eqnarray}
\label{eq:W1solve}\mathcal{W}^{[1]} &=& - \ii \ve^{-1} \ang{\momO}{0} - 2
\Ang{1}{\dx \mom{1}{1}} +  \Frac{1}{24}  \ii \dt^2 \ve  [[ \ang{\momO}{0} ,\ang{1}{2}], \ang{1}{2}] \\
\nonumber &&+ \Frac{1}{12} \dt^2  \ve [[ \Ang{1}{\dx \mom{1}{1}},\ang{1}{2}],
\ang{1}{2}]
- \Frac{1}{12} \ii \dt   \ve^{-1} [[ \ang{\momO}{0}, \ang{1}{2}],  \ang{\momO}{0}]\\
\nonumber &&- \Frac{1}{6} \dt [[\ang{\momO}{0}, \ang{1}{2}],\Ang{1}{\dx
\mom{1}{1}}] - \Frac{1}{6}\dt  [[
\Ang{1}{\dx \mom{1}{1}}, \ang{1}{2}], \ang{\momO}{0}]\\
\nonumber && + \Frac{1}{3}\ii  \dt \ve   [[ \Ang{1}{\dx \mom{1}{1}},
\ang{1}{2}], \Ang{1}{\dx \mom{1}{1}}] + \O{h^5 \ve^{-1}},
\end{Eqnarray}
and we have ignored all $\O{h^5\ve^{-1}}=\O{\ve^{5\sigma-1}}$ terms in the
sBCH since we are applying the Zassenhaus splitting to the fourth-order
Magnus expansion.

%Since $\momO = \O{h}$ and $\mom{1}{1} = \O{h^3}$, and all commutators are
%$\O{\ve^{-1}}$ or smaller due to Theorem~\ref{thm:ve}, we find that the only
%commutators  that need to be solved for an $\O{h^5 \ve^{-1}}$ accuracy are .

Further, we observe that
\begin{Eqnarray}
\label{eq:W1solve2}\mathcal{W}^{[1]} &=& - \ii \ve^{-1} \ang{\momO}{0} - 2
\Ang{1}{\dx \mom{1}{1}} +  \Frac{1}{24}  \ii \dt^2 \ve  [[ \ang{\momO}{0} ,\ang{1}{2}], \ang{1}{2}] \\
\nonumber && - \Frac{1}{12} \ii \dt   \ve^{-1} [[ \ang{\momO}{0},
\ang{1}{2}],  \ang{\momO}{0}] + \O{h^5 \ve^{-1}},
\end{Eqnarray}
since most commutators are $\O{h^5 \ve^{-1}}$ or smaller due to
Theorem~\ref{thm:ve} and the observation that $\momO = \O{h}$ and $\mom{1}{1}
= \O{h^3}$.
%Further, we observe that all commutators with the exception of $[[
%\ang{\momO}{0} ,\ang{1}{2}], \ang{1}{2}] $ and $[[ \ang{\momO}{0},
%\ang{1}{2}], \ang{\momO}{0}]$ in \R{eq:W1solve} are $\O{h^5 \ve^{-1}}$ or
%smaller due to Theorem~\ref{thm:ve} and the observation that $\momO = \O{h}$
%and $\mom{1}{1} = \O{h^3}$.
%
%Substituting $X$ and $Y$\footnote{\Ac{Note: ONLY two commutators needed to be
%computed here! We did a massive overkill! We needed to compute only $[[
%\ang{\momOS{e}}{0} ,\ang{1}{2}], \ang{1}{2}] $ and $[[ \ang{\momOS{e}}{0},
%\ang{1}{2}], \ang{\momOS{e}}{0}]$. The rest are $\O{h^5}$ because of the
%above logic and
%we can immediately discard. %In fact, check out $\mathcal{W}^{[1]}$ in the
%next page, ordered in powers of $h$. Half of it is redundant. The good thing
%is that we would need half of this in the case of $\Theta_4$, so it is not a
%complete waste, but this particular part of $\Theta_2$ can be MUCH easier.
%MOREOVER, when we take $N$ into account, these terms might matter again since
%powers of $h$ are not everything!! So maybe we stick with this and say... we
%can discard at this stage, but for demonstrative purposes and for future use,
%we do everything, including terms that are very small. We really need to
%think about $h,N$ again.
%}}, we conclude that
%fully worked out
%\begin{Eqnarray*}
%[\ang{\momOS{e}}{0} ,\ang{1}{2}] & = & - 2 \ang{\dx \momOS{e}}{1}, \\
%\left[ \left[\ang{\momOS{e}}{0} ,\ang{1}{2}\right], \ang{1}{2}\right] & = & - 2 [\ang{\dx \momOS{e}}{1}, \ang{1}{2}] \\
%&=& 4 \ang{\dx^2 \momOS{e}}{2} -  \ang{\dx^4 \momOS{e}}{0},\\
%\left[ \Ang{1}{\dx \momS{o}{1}{1}},\ang{1}{2}\right] &= & - 2\ang{\dx^2  \momS{o}{1}{1} }{2} + \Frac12 \ang{\dx^4 \momS{o}{1}{1}}{0},\\
%\left[\left[ \Ang{1}{\dx \momS{o}{1}{1}},\ang{1}{2}\right], \ang{1}{2}\right] &=&
%-2 [\ang{\dx^2  \momS{o}{1}{1} }{2},\ang{1}{2}] + \Frac12 [\ang{\dx^4 \momS{o}{1}{1}}{0}, \ang{1}{2}]\\
%&=& 4 \ang{\dx^3 \momS{o}{1}{1}}{3} -3 \ang{\dx^5 \momS{o}{1}{1}}{1},\\
%\left[ \left[ \ang{\momOS{e}}{0}, \ang{1}{2}\right],  \ang{\momOS{e}}{0}\right] & = & -2 [\ang{\dx \momOS{e}}{1}, \ang{\momOS{e}}{0}]= -2 \ang{(\dx \momOS{e})^2}{0}\\
%\left[ \left[\ang{\momOS{e}}{0},
%\ang{1}{2}\right],\Ang{1}{\dx\momS{o}{1}{1}}\right] & = & - 2 \left[ \ang{\dx
%\momOS{e}}{1} ,\Ang{1}{\dx\momS{o}{1}{1}}\right]\\
%&=& -2 \ang{(\dx \momOS{e}) (\dx^2 \momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx
%\momS{o}{1}{1})}{1}\\
%\left[ \left[ \Ang{1}{\dx \momS{o}{1}{1}}, \ang{1}{2}\right],
%\ang{\momOS{e}}{0}\right] &=& \left[ - 2\ang{\dx^2  \momS{o}{1}{1} }{2} +
%\Frac12 \ang{\dx^4 \momS{o}{1}{1}}{0},\ang{\momOS{e}}{0}\right]\\
%&=& -4 \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\\
%\left[ \left[ \Ang{1}{\dx \momS{o}{1}{1}}, \ang{1}{2}\right], \Ang{1}{\dx
%\momS{o}{1}{1}}\right] &= & \left[ - 2\ang{\dx^2  \momS{o}{1}{1} }{2} +
%\Frac12 \ang{\dx^4 \momS{o}{1}{1}}{0},  \Ang{1}{\dx \momS{o}{1}{1}}\right]\\
%&=& - 2 \ang{2 (\dx^2  \momS{o}{1}{1})^2 - (\dx^3
%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2}\\
%&& + \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2 \momS{o}{1}{1}) (\dx^4
%\momS{o}{1}{1})}{0} \\
%&& -\Frac12 \ang{(\dx \momS{o}{1}{1})(\dx^5 \momS{o}{1}{1})}{0}.
%\end{Eqnarray*}
These nested commutators can be simplified using the identities \R{eq:id},
the detailed theory for which is presented in \cite{psalgebra} and which were
utilised in the derivation of the simplified-commutator Magnus expansion
$\Theta_2$ in \cite{IKS18sinum}. Applying these identities, we find
\begin{Eqnarray}
\label{eq:commutators} [\ang{\momO}{0} ,\ang{1}{2}] & = & - 2 \ang{\dx \momO}{1}, \\
\nonumber\left[ \left[\ang{\momO}{0} ,\ang{1}{2}\right], \ang{1}{2}\right] & = &  4 \ang{\dx^2 \momO}{2} -  \ang{\dx^4 \momO}{0},\\
\nonumber \left[ \Ang{1}{\dx \mom{1}{1}},\ang{1}{2}\right] &= & - 2\ang{\dx^2  \mom{1}{1} }{2} + \Frac12 \ang{\dx^4 \mom{1}{1}}{0},\\
%\left[\left[ \Ang{1}{\dx \momS{o}{1}{1}},\ang{1}{2}\right], \ang{1}{2}\right]
%\nonumber &=& 4 \ang{\dx^3 \momS{o}{1}{1}}{3} -3 \ang{\dx^5
%\momS{o}{1}{1}}{1}.\\
\nonumber \left[ \left[ \ang{\momO}{0}, \ang{1}{2}\right],
\ang{\momO}{0}\right] & = &  -2 \ang{(\dx \momO)^2}{0}.
%\\
%\left[ \left[\ang{\momOS{e}}{0}, \nonumber \nonumber
%\ang{1}{2}\right],\Ang{1}{\dx\momS{o}{1}{1}}\right] & = & -2 \ang{(\dx
%\momOS{e}) (\dx^2 \momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx
%\momS{o}{1}{1})}{1}
%\\
%\left[ \left[ \Ang{1}{\dx \momS{o}{1}{1}}, \ang{1}{2}\right],
%\nonumber \ang{\momOS{e}}{0}\right] &=&  -4 \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\\
%\left[ \left[ \Ang{1}{\dx \momS{o}{1}{1}}, \ang{1}{2}\right], \Ang{1}{\dx
%\nonumber \momS{o}{1}{1}}\right] &= &  - 2 \ang{2 (\dx^2  \momS{o}{1}{1})^2 -
%(\dx^3
%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2}\\
%\nonumber && + \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2 \momS{o}{1}{1})
%(\dx^4
%\momS{o}{1}{1})}{0} \\
%\nonumber && -\Frac12 \ang{(\dx \momS{o}{1}{1})(\dx^5 \momS{o}{1}{1})}{0}.
\end{Eqnarray}
%
%
%% intermediate workings:
%%\begin{Eqnarray*}
%%\mathcal{W}^{[1]} &=& - \ii  \momOS{e} - 2
%%\Ang{1}{\dx \momS{o}{1}{1}} +  \ii \dt^2 \Frac{1}{24} \left(4 \ang{\dx^2 \momOS{e}}{2} -  \ang{\dx^4 \momOS{e}}{0} \right) \\
%%&&+ \dt^2 \Frac{1}{12} \left( 4 \ang{\dx^3 \momS{o}{1}{1}}{3} -3 \ang{\dx^5
%%\momS{o}{1}{1}}{1} \right)
%%- \ii \dt  \Frac{1}{12} \left( -2 \ang{(\dx \momOS{e})^2}{0}\right)\\
%%&&-  \dt\Frac{1}{6} \left(-2 \ang{(\dx \momOS{e}) (\dx^2
%%\momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx \momS{o}{1}{1})}{1}\right) \\
%%&&-
%%\dt\Frac{1}{6} \left(-4 \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\right)\\
%%&& + \ii \dt\Frac{1}{3}  \left( - 2 \ang{2 (\dx^2  \momS{o}{1}{1})^2 - (\dx^3
%%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2} \right.\\
%%&&\qquad \quad+ \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2 \momS{o}{1}{1})
%%(\dx^4
%%\momS{o}{1}{1})}{0}\\
%%&&\qquad \quad\left. -\Frac12 \ang{(\dx \momS{o}{1}{1})(\dx^5
%%\momS{o}{1}{1})}{0}\right).
%%\end{Eqnarray*}
%
%
%%intermediate: brackets opened
%%\begin{Eqnarray*}
%%\mathcal{W}^{[1]} &=& - \ii  \momOS{e} - 2 \Ang{1}{\dx \momS{o}{1}{1}} +  \ii
%%\dt^2 \Frac{1}{6}  \ang{\dx^2 \momOS{e}}{2}  -  \ii \dt^2 \Frac{1}{24}
%%\ang{\dx^4 \momOS{e}}{0}\\
%%&&+ \dt^2 \Frac{1}{3}  \ang{\dx^3 \momS{o}{1}{1}}{3} -\dt^2 \Frac{1}{4}
%%\ang{\dx^5 \momS{o}{1}{1}}{1}
%%+\ii \dt  \Frac{1}{6} \ang{(\dx \momOS{e})^2}{0}\\
%%&&+ \dt\Frac{1}{3}  \ang{(\dx \momOS{e}) (\dx^2
%%\momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx \momS{o}{1}{1})}{1} \\
%%&&+
%%\dt\Frac{2}{3} \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\\
%%&& - \ii \dt\Frac{2}{3}   \ang{2 (\dx^2  \momS{o}{1}{1})^2 - (\dx^3
%%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2}\\
%%&&\qquad \quad+ \ii \dt\Frac{1}{3} \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2
%%\momS{o}{1}{1}) (\dx^4
%%\momS{o}{1}{1})}{0}\\
%%&&\qquad \quad -\ii \dt\Frac{1}{6} \ang{(\dx \momS{o}{1}{1})(\dx^5
%%\momS{o}{1}{1})}{0}.
%%\end{Eqnarray*}
%Using \R{eq:commutators} and
%Recalling from Sections~\ref{sec:powersofh_oddeven_mu_lambda} and
%\ref{sec:extracting_odd_Magnus} that
%\[\momOS{e} = \O{h}, \quad \momS{o}{1}{1} = \O{h^3},\]
%we conclude that
%rewritten in rcases style with right bracket
%\begin{Eqnarray*}
%\mathcal{W}^{[1]} &=& \Ac{\O{h}} - \ii  \momOS{e} \\
%&& \Ac{\O{h^3}} + \ii \dt^2 \Frac{1}{6} \ang{\dx^2 \momOS{e}}{2} - 2
%\Ang{1}{\dx \momS{o}{1}{1}}  \\
%&&-  \ii \dt^2 \Frac{1}{24}
%\ang{\dx^4 \momOS{e}}{0}+\ii \dt  \Frac{1}{6} \ang{(\dx \momOS{e})^2}{0}\\
%&&\Ac{\O{h^5}}+ \dt^2 \Frac{1}{3}  \ang{\dx^3 \momS{o}{1}{1}}{3} -\dt^2
%\Frac{1}{4} \ang{\dx^5 \momS{o}{1}{1}}{1}\\
%&&+ \dt\Frac{1}{3}  \ang{(\dx \momOS{e}) (\dx^2
%\momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx \momS{o}{1}{1})}{1} \\
%&&+
%\dt\Frac{2}{3} \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\\
%&& \Ac{\O{h^7}}- \ii \dt\Frac{2}{3}   \ang{2 (\dx^2  \momS{o}{1}{1})^2 -
%(\dx^3
%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2}\\
%&&\qquad \quad+ \ii \dt\Frac{1}{3} \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2
%\momS{o}{1}{1}) (\dx^4
%\momS{o}{1}{1})}{0}\\
%&&\qquad \quad -\ii \dt\Frac{1}{6} \ang{(\dx \momS{o}{1}{1})(\dx^5
%\momS{o}{1}{1})}{0}.
%\end{Eqnarray*}
%\begin{equation}
%\begin{split}
%%O(h)
%&\begin{rcases}
%\mathcal{W}^{[1]} &= - \ii  \momOS{e} \qquad \qquad \\
%\end{rcases}  {\O{h}}\\
%%O(h^3)
%&\qquad\quad\begin{rcases} \noalign{\vskip2pt} & + \ii \dt^2 \Frac{1}{6}
%\ang{\dx^2 \momOS{e}}{2} - 2
%\Ang{1}{\dx \momS{o}{1}{1}}  \\
%&-  \ii \dt^2 \Frac{1}{24}
%\ang{\dx^4 \momOS{e}}{0}+\ii \dt  \Frac{1}{6} \ang{(\dx \momOS{e})^2}{0}\\
%\end{rcases}  {\O{h^3}}\\
%%O(h^5)
%&\qquad\quad\begin{rcases}
%\noalign{\vskip2pt}
%&+ \dt^2 \Frac{1}{3}  \ang{\dx^3 \momS{o}{1}{1}}{3} -\dt^2
%\Frac{1}{4} \ang{\dx^5 \momS{o}{1}{1}}{1}\\
%&+ \dt\Frac{1}{3}  \ang{(\dx \momOS{e}) (\dx^2
%\momS{o}{1}{1})-(\dx^2 \momOS{e})(\dx \momS{o}{1}{1})}{1} \\
%&+
%\dt\Frac{2}{3} \ang{(\dx^2  \momS{o}{1}{1}) (\dx \momOS{e})}{1}\\
%\end{rcases}  {\O{h^5}}\\
%%O(h^7)
%&\qquad\quad\begin{rcases}
%\noalign{\vskip2pt}
%& - \ii \dt\Frac{2}{3}   \ang{2 (\dx^2  \momS{o}{1}{1})^2 -
%(\dx^3
%\momS{o}{1}{1}) (\dx \momS{o}{1}{1})}{2}\\
%&\qquad \quad+ \ii \dt\Frac{1}{3} \ang{2(\dx^3  \momS{o}{1}{1})^2 + (\dx^2
%\momS{o}{1}{1}) (\dx^4
%\momS{o}{1}{1})}{0}\\
%&\qquad \quad -\ii \dt\Frac{1}{6} \ang{(\dx \momS{o}{1}{1})(\dx^5
%\momS{o}{1}{1})}{0}.
%\end{rcases}  {\O{h^7}}
%\end{split}
%\end{equation}
%\footnote{A careful reader would note that, considering the respective sizes
%of $\momOS{e}$ and $\momS{o}{1}{1}$, we could do away with many commutators
%in the computation of $\mathcal{W}^{[1]}$ at the outset. In the development
%of certain variants of the Zassenhaus splitting, however, these terms will
%prove helpful. This forms the motivation of showing the algebraic
%computations in full here.}
%Once again, all $\O{h^5}$ terms can be safely
%discarded in the derivation of the Zassenhaus splitting since $\Theta_{2}$
%already involves a local error of $\O{h^5}$.
Thus, the central exponent in \R{eq:3:sbch_inverted} up to $\O{h^5
\ve^{-1}}=\O{\ve^{5\sigma-1}}$ is
\begin{Eqnarray}\label{eq:3:central_exponent}
\mathcal{W}^{[1]} &=&  - \ii \ve^{-1}  \ang{\momO}{0} +  \Frac{1}{6} \ii
\dt^2 \ve \ang{\dx^2
\momO}{2} - 2 \Ang{1}{\dx \mom{1}{1}}\\
\nonumber && -  \Frac{1}{24} \ii \dt^2  \ve \ang{\dx^4 \momO}{0}+\Frac{1}{6}
\ii \dt \ve^{-1}
 \ang{(\dx \momO)^2}{0}.
\end{Eqnarray}
In order to approximate the exponential of $\mathcal{W}^{[1]}$ (which is
required in \R{eq:3:sbch_inverted}), we apply the sBCH again along the lines
of \R{eq:3:sbch_inverted}, writing
\begin{equation}\label{eq:4:sbch_inverted}
  \ee^{\mathcal{W}^{[1]}} =\ee^{-\frac12  \ii \ve^{-1} \momO} \ee^{\mathcal{W}^{[2]} } \ee^{-\frac12  \ii \ve^{-1} \momO} + \O{h^5\ve^{-1}}.
\end{equation}
Here we have chosen to extract the largest term $X = W^{[1]} = - \ii \ve^{-1}
\momO = \O{h\ve^{-1}}$ and the remainder is $Y = \mathcal{W}^{[1]}- W^{[1]} =
\O{h^3\ve^{-1}}$. The choice of X is more obvious in this case since there is
only one term of size $\O{h\ve^{-1}}$. Keeping the sizes of $X$ and $Y$ in
mind, we find that
\begin{Eqnarray} \label{eq:4:central_exponent}
\nonumber \mathcal{W}^{[2]} &:=& \CC{sBCH}(-X,X+Y)+ \O{h^5 \ve^{-1}} = (-X + (X+Y)) = Y + \O{h^5 \ve^{-1}}\\
&=& \Frac{1}{6} \ii \dt^2 \ve \ang{\dx^2 \momO}{2} - 2 \Ang{1}{\dx
\mom{1}{1}}\\
\nonumber && \mbox{}-  \Frac{1}{24}\ii \dt^2 \ve \ang{\dx^4 \momO}{0}+\Frac{1}{6}
\ii \dt \ve^{-1}
 \ang{(\dx \momO)^2}{0} + \O{h^5 \ve^{-1}}
\end{Eqnarray}
suffices up to $\O{h^5 \ve^{-1}}$ since $[[Y,X],X]$ and $[[Y,X],Y]$ are
$\O{h^5\ve^{-1}}$ and $\O{h^7\ve^{-1}}$, respectively. Further, we discard
the $\O{h^3 \ve}$ term $-  \Frac{1}{24}\ii \dt^2 \ve \ang{\dx^4 \momO}{0}$
from \R{eq:4:central_exponent} since, under the assumption $\sigma \leq 1$,
it is effectively $\O{\ve^{5\sigma-1}}$ or smaller.

Finally, we complete the derivation of our fourth-order Magnus--Zassenhaus
splitting by combining \R{eq:3:sbch_inverted} and \R{eq:4:sbch_inverted},
\begin{equation}
\label{eq:MZ2}
	 \exp(\Theta_{2}) = \ee^{\frac12 W^{[0]}} \ee^{\frac12 W^{[1]}}
									 \ee^{\WW^{[2]}} \ee^{\frac12 W^{[1]}} \ee^{\frac12 W^{[0]}} + \O{\ve^{5\sigma-1}},
\end{equation}
which has the same form as the splittings described in
Appendix~\ref{sec:Zassenhaus}. Here the exponents (chosen and/or computed
during the derivation) are
\begin{Eqnarray}
W^{[0]} & = & \ii \dt \ve \dx^2  = \O{\ve^{\sigma-1}},\label{eq:MZ2W} \\
W^{[1]} & = & - \ii  \ve^{-1}  \momO = \O{\ve^{\sigma-1}}, \nonumber\\
\WW^{[2]} & = & \Frac{1}{6}\ii  \dt \ve^{-1} \left(\dx \momO \right)^2
-2\Ang{1}{\dx \mom{1}{1}}+\Frac{1}{6}\ii  \dt^2 \ve \Ang{2}{\dx^{2} \momO } =
\O{\ve^{3\sigma-1}}.\nonumber
\end{Eqnarray}

It is only by this stage -- having arrived at an asymptotic splitting
expressed in operatorial terms -- that we start considering discretisation
issues. Apart from analysis of size, considerations of spatial and temporal
discretisation (in the form of approximation through quadrature) are entirely
independent of the procedure leading to \R{eq:MZ2W} and of each other: one may proceed to address them in any order.


\begin{remark}
Note that, in contrast to the Magnus--Zassenhaus splitting of \cite{BIKS},
our exponents retain the integrals intact (in $\momO$ and $\mom{1}{1}$). This
provides us with the flexibility to choose the most suitable approximation method
 including the possibility of analytic approximations. This
flexibility proves particularly helpful in the case of potentials with high
temporal oscillations.
\end{remark}

%which incurs an error of $\O{\ve^{5\sigma -1}}$.
\begin{remark}
As a quick sanity check, we do arrive at the standard symmetric Zassenhaus
splitting \cite{bader14eaf} for time-independent potentials, $V(x,t) :=
V(x)$.
\end{remark}

\subsection{Implementation}

\label{sec:MZ2implementation} The operatorial splitting given by \R{eq:MZ2}
and \R{eq:MZ2W} can be converted into a concrete numerical scheme by
resorting to spatial discretisation. As typical, we use spectral collocation,
whereby $W^{[0]}$ is discretised as the circulant matrix $\widetilde{W^{[0]}}
= \ii \dt \ve \K_2$. Note that $\K_2$ is diagonalisable via Fourier transform
since
\begin{equation}
\label{eq:KkFFT}
\K_k = \FFF^{-1} \DDD_{c_k} \FFF,
\end{equation}
where $c_k$ is the
symbol of $\K_k$, $\FFF$ is the Fast Fourier Transform (FFT) and $\FFF^{-1}$
is its inverse (IFFT). Thus, we can evaluate
\[
\ee^{\frac12 \widetilde{W^{[0]}}} \MM{u}  = \mathcal{F}^{-1} \DDD_{\exp(\frac12 \ii \dt \ve c_2)} \mathcal{F} \MM{u},
\]
in $\O{N \log N}$ operations. The next exponent, $W^{[1]}$, is discretised as
the diagonal matrix $\widetilde{W^{[1]}} = - \ii \ve^{-1} \DDD_{\momO}$ and
exponentiated pointwise in $\O{N}$ operations,
\[
\ee^{\frac12 \widetilde{W^{[1]}}} \MM{u} = \DDD_{\exp(\frac12 \ii \ve^{-1} \momO)} \MM{u}.
\]
Lastly, the innermost exponent,
\begin{Eqnarray*}
\WW^{[2]} \leadsto  \widetilde{\WW^{[2]}} & = & \Frac{1}{6}\ii  \dt \ve^{-1}
\DDD_{\left(\dx \momO \right)^2} +\left(\K_1 \DDD_{\dx \mom{1}{1}}+ \DDD_{\dx
\mom{1}{1}}\K_1\right)\\
&&-\Frac{1}{3}\ii \dt^2 \ve \left(\K_2 \DDD_{\dx^{2} \momO } + \DDD_{\dx^{2}
\momO } \K_2\right),
\end{Eqnarray*}
which is neither circulant nor diagonal, can be very effectively
exponentiated via Lanczos iterations because (unlike the first two exponents)
it is very small in size, even when combined with large time steps.

For instance, when using time steps as large as $h = \O{\ve^{1/2}}$, i.e.\
under the scaling $\sigma = 1/2$, the exponent $\widetilde{\WW^{[2]}}$ is
$\O{\ve^{1/2}}$. As the semiclassical parameter $\ve \ll 1$ becomes small,
this spectral radius approaches $0$. Thus the superlinear accuracy of Lanczos
iterations is seen immediately and merely four Lanczos iterations are required
for an exponentiation to an accuracy of $\O{\ve^{5\sigma-1}}=\O{\ve^{3/2}}$,
which is the accuracy of the splitting. A more detailed analysis of the
number of Lanczos iterations required for such exponents is carried out in
\cite{bader14eaf,BIKS}.
%
% As a matter of fact, we require merely two Lanczos iterations in
%order to approximate the exponential to an accuracy of $\O{\ve^{5\sigma-1}}$.
%A detailed analysis is carried out in \cite{bader14eaf,BIKS}.

Each Lanczos iteration requires the computation of a matrix--vector product
of the form $\widetilde{\WW^{[2]}} \MM{v}$. In general Lanczos iterations for
the discretisation of $W = \sum_{k=0}^n \ii^{k+1} \ang{f_k}{k}$ to
$\widetilde{W} = \ii \DDD_{f_0} + \frac12 \sum_{k=1}^n \ii^{k+1}
\left(\DDD_{f_k} \K_k +\K_k \DDD_{f_k} \right)$ can be efficiently computed
in $2n+2$ Fast Fourier Transforms (included inverses) using the expression
 \begin{Eqnarray}
\label{eq:Wv}  \widetilde{W}\MM{v} = \ii \DDD_{f_0} \MM{v} + \Frac12 \left(
\sum_{k=1}^n \ii^{k+1} \DDD_{f_k} \FFF^{-1} \DDD_{c_k} \right) \FFF \MM{v} +
\Frac12 \FFF^{-1} \left( \sum_{k=1}^n \ii^{k+1}  \DDD_{c_k} \FFF \DDD_{f_k}
\MM{v}\right).
\end{Eqnarray}
Thus, the computation of $\widetilde{\WW^{[2]}} \MM{v}$ in each Lanczos
iteration requires six FFTs and the total cost of its exponentiation is 24
FFTs. This completes the derivation of the splitting described in
\R{eq:Zass2}.

\begin{remark}
$\Theta_0$ is an order two Magnus expansion. An order two
Zassenhaus splitting is merely the Strang splitting. Thus an order two
Magnus--Zassenhaus splitting is, trivially, \R{eq:expmidpoint}, which has been
presented in the introduction.
\end{remark}

\begin{remark}
We assume that the integrals $\momO$ and $\mom{1}{1}$ are either available
analytically or can be adequately approximated via quadrature formulae such
as Gauss--Legendre quadratures, along the lines of \cite{IKS18sinum}.

%Some options for approximating integrals will be explored in
%Section~\ref{sec:numerics} for specific potentials.
\end{remark}

\begin{remark} Along the lines of \cite{BIKS,IKS18sinum}, we also assume that spatial derivatives of the potential, as well as
its integrals, are either available or inexpensive to compute.
\end{remark}
%
%\begin{equation}
%\begin{split}
%%O(h)
%&\begin{rcases}
%W^{[0]} &= \ii \dt \dx^2,\qquad \qquad \\
%\end{rcases}  {\O{h}}\\
%&\begin{rcases}
%W^{[1]} &= - \ii \momOS{e},\qquad \\
%\end{rcases}  {\O{h}}\\
%&\begin{rcases}
%\mathcal{W}^{[2]} &=  \ii \dt^2 \Frac{1}{6} \ang{\dx^2 \momOS{e}}{2} - 2
%\Ang{1}{\dx\momS{o}{1}{1}}\\
%& -  \ii \dt^2 \Frac{1}{24} \ang{\dx^4 \momOS{e}}{0}+\ii \dt\Frac{1}{6} \ang{(\dx \momOS{e})^2}{0}.
%\end{rcases}   {\O{h^3}}
%\end{split}
%\end{equation}


%
%All through, we discard terms smaller than our error tolerance -- for
%$\Omt{2p-1}$ this means discarding terms of size $\O{\ve^{(2p+1)\sigma -1}}$.
%For $\sOmt{3}$, where $p=2$, we get a five-stage splitting by starting with
%$X = \ii \dt \ve \dx^2$ and then extracting the largest term at each
%iteration,
%\begin{equation}
%\label{eq:Zass3}
%	\exp\left(\Omt{3}\right) = \ee^{\frac12 W^{[0]}} \ee^{\frac12 W^{[1]}} \ee^{\WW^{[2]}} \ee^{\frac12 W^{[1]}} \ee^{\frac12 W^{[0]}} + \O{\ve^{5 \sigma -1}},
%\end{equation}
%where


%\Ac{This does not hold for the full Magnus splitting -- something is wrong, terms are getting discarded incorrectly, clearly!!}.

%
%\subsection{Powers of $h$ and $N$} Analysing in powers of the time step $h$,
%as we have done in the previous sections, is an effective strategy for
%deriving Magnus expansions and splitting schemes for ODEs. When it comes to
%numerical schemes for PDEs, however, there is an interplay between the
%temporal and spatial grid resolutions that ought to be taken into account.
%Essentially, this interplay stems from the fact that an increase in the
%spatial resolution results in larger matrices, both in terms of dimension and
%norm. The increase in norm needs to be balanced by a suitably depressed time
%step in order for progressive terms in expansions such as the Magnus
%expansion to become smaller.
%
%Thus, a more realistic analysis of the size of the terms in a Magnus
%expansion such as \R{Theta_4} can be done by keeping in mind that terms of
%the form $\ang{f}{k}$ are eventually discretised as
%\begin{equation}
%\tag{\ref{eq:angbradisc}}
% \ang{f}{k} \leadsto \Frac12 \left( \DDD_f \K_k + \K_k \DDD_f \right).
%\end{equation}
%and noting that under spectral collocation or Fourier spectral
%discretisation,
%\begin{equation}
%    \norm{2}{\K_k} \leq \left(\frac{\pi N}{2}\right)^k, \quad \norm{2}{\DDD_f} \leq \norm{\infty}{f},
%\end{equation}
%where $N$ is the number of grid points. Consequenty, we may
%conclude\footnote{This involves a slight abuse of notation since $\ang{f}{k}$
%is an undiscretised and unbounded operator. More formally, the discretisation
%$\ang{f}{k} \leadsto B_N$ scales as $\norm{2}{B_N} \leq \norm{\infty}{f}
%\left(\frac{\pi N}{2}\right)^k$.} that upon discretisation the following
%scaling holds
%\begin{equation}
%\label{eq:sizeang}
% \ang{f}{k} \sim \norm{\infty}{f} \left(\frac{\pi N}{2}\right)^k = \O{\norm{\infty}{f} N^k}.
%\end{equation}
%As we have seen in the workings till now, the functions $f$ that appear in
%$\ang{f}{k}$ are integrals and derivatives of the potential \Ac{(see xyz
%eqns)}. In principle the derivatives of the potential could be growing or
%decreasing (or even vanishing) in different applications. Where the growth is
%substantial, taking this into account while designing an effective method
%(via the size estimate \R{eq:sizeang}) becomes important. Where these
%derivatives are mild, however, we may make the analysis simpler by absorbing
%$\norm{\infty}{f}$ into the constant,
%\begin{equation}
%\label{eq:sizeangN}
% \ang{f}{k} = \O{N^k},
%\end{equation}
%and analyse solely in powers of $N$. This is the strategy that we will pursue
%in the current section.
%
%Thus \R{eq:3:sbch_inverted} reads as
%\begin{equation}\label{eq:4:sbch_inverted}
%  \ee^{\Theta_{2}^o} =\ee^{\frac12 \ii \dt \dx^2} \ee^{ - \ii  \momOS{e} + \ii \dt^2 \Frac{1}{6}
%\ang{\dx^2 \momOS{e}}{2} - 2
%\Ang{1}{\dx \momS{o}{1}{1}} -  \ii \dt^2 \Frac{1}{24}
%\ang{\dx^4 \momOS{e}}{0}+\ii \dt  \Frac{1}{6} \ang{(\dx \momOS{e})^2}{0}} \ee^{\frac12  \ii \dt \dx^2} + \O{h^5}.
%\end{equation}
%In the second application of the sBCH formula, we want to split the central exponent in



%which can help us compute the sBCH in \R{eq:3:sbch_inverted} easily.  Thus,

%Since we are applying the Zassenhaus splitting to the fourth-order Magnus expansion, we can discard all $\O{h^5}$ terms.

